SUT: Active Defects Probing for Transcompiler Models

Automatic Program translation has enormous application value and hence has been attracting significant interest from AI researchers. However, we observe that current program translation models still make elementary syntax errors, particularly, when the target language does not have syntax elements in the source language. Metrics like BLUE, CodeBLUE and computation accuracy may not expose these issues. In this paper we introduce a new metrics for programming language translation and these metrics address these basic syntax errors. We develop a novel active defects probing suite called Syntactic Unit Tests (SUT) which includes a highly interpretable evaluation harness for accuracy and test scoring. Experiments have shown that even powerful models like ChatGPT still make mistakes on these basic unit tests. Specifically, compared to previous program translation task evaluation dataset, its pass rate on our unit tests has decreased by 26.15%. Further our evaluation harness reveal syntactic element errors in which these models exhibit deficiencies.

==> figs/defect_example.tex <==
\begin{figure}[t]
\center
\begin{adjustbox}{width=.8\linewidth}
\begin{tabular}{lp{20ex}}
\toprule
 & \multicolumn{1}{c}{Code}  \\
\midrule

Source C++  &
\begin{minipage}{\textwidth}
\begin{lstlisting}[language=C++,escapeinside=||]
int foo(int a) {
    int b = ++a;
    return b;
}
\end{lstlisting}
\end{minipage}\\

\midrule

Translated Python (TransCoder)  &
\begin{minipage}{\textwidth}
\begin{lstlisting}[language=Python,escapeinside=||]
def foo ( a ) :
    |\textcolor{red}{b = yield a}|
    return b
\end{lstlisting}
\end{minipage}\\

% \midrule
% Translated Python (TransCoder-ST)\qquad\qquad  &
% \begin{minipage}{\textwidth}
% \begin{lstlisting}[language=Python,escapeinside=||]
% def foo ( a ) :
%     |\textcolor{red}{b = a + 1}|
%     return b
% \end{lstlisting}
% \end{minipage}\\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
An example C++ source program and the Python translation predicted by Transcoder. 
%The prefix increment \texttt{++a} is not a syntax element of Python, and occurs infrequently enough in the data that TransCoder did not learn to correctly translate it.
}
\label{fig:defect_example}
\end{figure}


==> figs/sut_case.tex <==
\begin{figure}[t]
    \centering
    \begin{adjustbox}{width=\linewidth}
    \begin{tabular}{|p{15ex}|p{22ex}|p{8ex}|p{15ex}|}
    \hline
    \textbf{name} & \textbf{src} & \textbf{input} & \textbf{expected\_output} \\
    \hline
    prefix increment operator &
\begin{minipage}{\textwidth}
\begin{lstlisting}[language=C++,escapeinside=||]
int foo(int a) {
    int b = ++a;
    return b;
}
\end{lstlisting}
\end{minipage}
    & [1, 2, 3] & [2, 3, 4] \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{An C++ SUT case example for prefix increment operator.}
    %The source function is translated to a function in the target language, which takes each value of the input list and returns the corresponding output. The translated function is considered syntactically equivalent to the source function if its output is the same as the expected output.}
    \label{fig:sut_case}
\end{figure}

==> tables/sets_results.tex <==
\begin{table}[t]
    \centering
    \caption{SETS experiment results on TransCoder C++$\rightarrow$Python model. We only show the top 10 syntax elements due to space limitation.}
    
    \resizebox{.9\linewidth}{!}{
    \begin{tabular}{lc}
        \toprule
        Syntax Elements & Coefficients \\
        \midrule

\texttt{do} & 801.9 \\
\texttt{template} & 782.3 \\
\texttt{case} & 579.5 \\
\texttt{null} & 384.1 \\
\texttt{template\_function} & 341.2 \\
\texttt{signed} & 335.6 \\
\texttt{update\_expression} & 288.2 \\
\texttt{pointer\_expression} & 277.6 \\
\texttt{structured\_binding\_declarator} & 221.9 \\
\texttt{cast\_expression} & 202.1 \\
        \bottomrule
    \end{tabular}
    }

\label{table:sets_results}
\end{table}

==> tables/sut_dataset_statistics.tex <==
\begin{table}[t]
\centering

\caption{Statistics of the Syntactic Unit Test benchmark dataset for the four languages we considered: C++, Java, Python, and C\#. Average tokens count were computed with the TransCoder tokenizer for C++, Java and Python, and the PLBART tokenizer for C\#.}

\resizebox{.9\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
Language & Test Cases & Syntax elements & Avg. tokens \\
\midrule
C++ & 108 & 100 & 29.5 \\
Java & 63 & 62 & 22.1 \\
Python & 63 & 58 & 24.6 \\
C\# & 168 & 134 & 36.4 \\
\bottomrule
\end{tabular}
}
\label{tab:sut_dataset_statistics}
\end{table}

